OledFL: Unleashing the Potential of Decentralized Federated Learning via Opposite Lookahead Enhancement

Decentralized Federated Learning (DFL) surpasses Centralized Federated Learning (CFL) in terms of faster training, privacy preservation, and light communication, making it a promising alternative in the field of federated learning. However, DFL still exhibits significant disparities with CFL in terms of generalization ability such as rarely theoretical understanding and degraded empirical performance due to severe inconsistency. In this paper, we enhance the consistency of DFL by developing an opposite lookahead enhancement technique (Ole), yielding OledFL to optimize the initialization of each client in each communication round, thus significantly improving both the generalization and convergence speed. Moreover, we rigorously establish its convergence rate in non-convex setting and characterize its generalization bound through uniform stability, which provides concrete reasons why OledFL can achieve both the fast convergence speed and high generalization ability. Extensive experiments conducted on the CIFAR10 and CIFAR100 datasets with Dirichlet and Pathological distributions illustrate that our OledFL can achieve up to 5\% performance improvement and 8$\times$ speedup, compared to the most popular DFedAvg optimizer in DFL.

==> tex/bio.tex <==

\vspace{-1cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/qinglunli.png}}]{Qinglun Li}
obtained his bachelor’s degree in Science from the School of Science at the University of Shanghai for Science and Technology. He is pursuing a doctorate in Management Science and Engineering at the National University of Defense Technology. His research interests include machine learning, decentralized federated learning, and non-convex optimization. He has served as ICML 2024 reviewer.
% \vspace{-1cm}
\end{IEEEbiography}
\vspace{-1cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in, clip,keepaspectratio]{bio/zhangmiao.jpg}}]{Miao Zhang} is currently a research assistant at National University of Defense Technology, Changsha, China. He received his bachelor’s degree from the School of Information, University of Science and Technology of China in 2015, and received his master’s degree and Ph.D. from the College of Systems Engineering, National University of Defense Technology in 2017 and 2022, respectively. His research interests include intelligence optimization, resource management, private computing, federated learning and reinforcement learning.
\end{IEEEbiography}
\vspace{-1cm}

\begin{IEEEbiography}[{\includegraphics[width=1.2in,height=1.25in,clip,keepaspectratio]{bio/mengzhu.pdf}}]{Mengzhu Wang}
 received the Master's degree from Chongqing University, Chongqing,~China, in 2018. From 2019 to 2023, she received the Ph.D. degree with the Science and Technology on Parallel and Distributed Laboratory, School of Computer Science, National University of Defense Technology, Changsha, China. She is currently an associate professor in Hebei University of Technology. Her current research interest include transfer learning and computer vision.
\end{IEEEbiography}
\vspace{-1cm}



\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in, clip,keepaspectratio]{bio/quanjun.pdf}}]{Quanjun yin} is currently a professor with the College of Systems Engineering, National University of Defense Technology, China. His research interests include cognitive process modelling, qualitative spatial reasoning and planning, cooperation and negotiation, cloud-based simulation, and edge computing.
\end{IEEEbiography}

\vspace{-1cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/li_shen.png}}]{Li Shen} is currently an associate professor at Sun Yat-sen University. Previously, he was a research scientist at JD Explore Academy, Beijing, and a senior researcher at Tencent AI Lab, Shenzhen. He received his bachelor's degree and Ph.D. from the School of Mathematics, South China University of Technology. His research interests include theory and algorithms for nonsmooth convex and nonconvex optimization, and their applications in trustworthy artificial intelligence, deep learning, and reinforcement learning. He has published more than 100 papers in peer-reviewed top-tier journal papers (JMLR, IEEE TPAMI, IJCV, IEEE TSP, IEEE TIP, IEEE TKDE, etc.) and conference papers (ICML, NeurIPS, ICLR, CVPR, ICCV, etc.). He has also served as the senior program committee for AAAI 2022, and AAAI 2024 and area chairs for ICML 2024, ICLR 2024, ICPR 2022, and ICPR 2024.
% \vspace{-1cm}
\end{IEEEbiography}


